Everything You Always Wanted to Know About TREC RTS* (*But Were Afraid to Ask)

The TREC Real-Time Summarization (RTS) track provides a framework for evaluating systems monitoring the Twitter stream and pushing tweets to users according to given profiles. It includes metrics, files, settings and hypothesis provided by the organizers. In this work, we perform a thorough analysis of each component of the framework used in 2016 and 2017 and found some limitations for the Scenario A of this track. Our main findings point out the weakness of the metrics and give clear recommendations to fairly reuse the collection.

==> sections/objectives.tex <==
\section{Formal constraints on evaluation metrics for RTS}
\textit{=>Yoann}

\subsection{Notations}


\subsection{Hypothesis and constraint}

\subsection{Expected properties}




Axiome forcément vérifié par tous les systèmes car contrainte de la tâche.


The task of automatically monitoring document streams to keep the user notified up to date on its topics of interest should consider several aspects.

Tackling such a task raises different issues:
\begin{enumerate}
\item do not overwhelm the user. The user does not want to receive too much notifications during a time period, however he/she wants interesting notifications.
\item do not notify the user too late. Being the first to inform is essential~\cite{Takemura2012}. The interest of an information decreases as time passes.
\item do not fail to deliver crucial information. The user does not want to miss important information except maybe if he/she is overwhelmed yet. 
\end{enumerate}

A system addressing this task should on pay attention to various criteria related to these issues: relevance, redundancy, coverage, latency, and overwhelming.

SETUP de l'évaluation / pré-requis : pas plus de 10 par jours (impossible pour le système de renvoyer plus)

With regard to each of these criteria, several objectives should be reached:
\begin{itemize}
\item Two objectives are aimed with respect to \textbf{relevance}:
    \begin{description}
        \item[R1.] The user prefers to receive relevant tweets (and less irrelevant tweets as possible). % P1
        \item[R2.] With the same number of relevant tweets, the user prefers less irrelevant tweets as possible.
        %\item[R2.] The user prefers to receive highly relevant tweets (rather than relevant ones). % P7
    \end{description}
\item \textbf{Redundancy/Verbosity} implies reaching the following objectives:
    \begin{description}
       % \item[V1.] The user prefers to receive less tweets as possible for each cluster. %R4
        \item[V1.] With the same number of clusters, the user prefers to receive less relevant tweets as possible. %R6 = R4 ?
    \end{description}
\item One objective relates to \textbf{coverage}:
    \begin{description}
        \item[C1.] The user prefers to receive tweets relating to different clusters. %C2
    \end{description}
\item Two objectives are aimed with respect to \textbf{latency}:
    \begin{description}
        \item[L1.] The user prefers to receive relevant information since the first time windows of its appearance. %L3
        \item[L2.] In a window, the user wants a relevant tweet as close as possible as the information appearance in the cluster, i.e., the beginning of the window. %L3'
    \end{description}
\item \textbf{Overwhelming} implies the two following objectives:
    \begin{description}
        \item[O1.] The user prefers not to exceed a maximum number of tweets per window. %S5
        \item[O2.] With the same found clusters, the user prefers to receive less irrelevant tweets as possible. %S6'
    \end{description}
\end{itemize}

With regard to these objectives, different cases have to be considered to evaluate the differences of performance between different systems, depending on which tweets are delivered and depending on their order of delivery.





NE PAS OUBLIER DE DIRE QU'ON FAIT LA SIMPLIFICATION TRES PERTINENT = PERTINENT

+ ON CONSIDERE TOUS LES CLUSTERS EGAUX
